LLM-based Weak Supervision Framework for Query Intent Classification in Video Search

Streaming services have reshaped how we discover and engage with digital entertainment. Despite these advancements, effectively understanding the wide spectrum of user search queries continues to pose a significant challenge. An accurate query understanding system that can handle a variety of entities that represent different user intents is essential for delivering an enhanced user experience. We can build such a system by training a natural language understanding (NLU) model; however, obtaining high-quality labeled training data in this specialized domain is a substantial obstacle. Manual annotation is costly and impractical for capturing users' vast vocabulary variations. To address this, we introduce a novel approach that leverages large language models (LLMs) through weak supervision to automatically annotate a vast collection of user search queries. Using prompt engineering and a diverse set of LLM personas, we generate training data that matches human annotator expectations. By incorporating domain knowledge via Chain of Thought and In-Context Learning, our approach leverages the labeled data to train low-latency models optimized for real-time inference. Extensive evaluations demonstrated that our approach outperformed the baseline with an average relative gain of 113% in recall. Furthermore, our novel prompt engineering framework yields higher quality LLM-generated data to be used for weak supervision; we observed 47.60% improvement over baseline in agreement rate between LLM predictions and human annotations with respect to F1 score, weighted according to the distribution of occurrences of the search queries. Our persona selection routing mechanism further adds an additional 3.67% increase in weighted F1 score on top of our novel prompt engineering framework.

==> Sections_Farnoosh/Customer_statement.tex <==
Once our model is deployed, it will play a crucial role in enhancing the customer experience for our Prime Video users. Accurately determining the intent behind customers' queries will enable our downstream systems to provide highly relevant search results and tailored experiences that align with the customers' specific needs and queries, ultimately leading to improved customer satisfaction. A failure in accurately determining query intent could result in the downstream systems providing non-relevant search results and experiences, potentially leading to decreased customer satisfaction with Prime Video. Although we  capture all entities in the head queries, we acknowledge the possibility of missing some entities in the tail queries due to the emergence of new queries or variations. Consequently, users may encounter instances where they do not receive very relevant results.

==> Sections_Farnoosh/data.tex <==
\section{Data}
% \subsection{Query Entities}

When exploring content on Prime Video, customers use a diverse range of search queries. They may search by offerType, such as "\textit{movies to rent}", or by audioLanguage, like "\textit{french movies}". They may also search based on releaseYear, for instance, "\textit{2023 TV show}", among many other criteria. We compiled a set of more than 20 entities that capture customer intent in their search. We provided the full entities, their explanations and examples in \ref{tab:entity_table}.

%The QU model is expected to support the following entities based on customer user stories: \texttt{IntentMovie}, \texttt{IntentTvSeries}, \texttt{Theme}, \texttt{Genre}, \texttt{Franchise}, \texttt{CastAndCrew}, \texttt{StreamingService}, \texttt{Holiday}, \texttt{Character}, \texttt{OfferType}, \texttt{ReleaseYear}, \texttt{Recency}, \texttt{Popularity}, \texttt{Decade}, \texttt{AudioLanguage}, \texttt{FreeContent}, \texttt{MovieName}, \texttt{TVSeriesName}, \texttt{Sport}, \texttt{LinearStation}, \texttt{Channels}.

% \subsection{Query Entities Breakdown for User Search Queries}

% To gain insights into user search behavior and preferences, we analyzed a dataset of 100,000 search queries, randomly sampled from a larger pool of the top one million unique popular user search queries. This broader dataset of one million queries was curated by capturing search logs from 14 randomly selected days in the first half of 2023 and another 14 random days in the second half of the year. To achieve precise data labeling, we leveraged Claude V2.1 along with fuzzy matching techniques. Figure~\ref{fig:entity_statistic} shows the proportion of each entity type present in the dataset. We further analyzed the search queries based on the total number of entities referenced. Non-title queries refer to queries that do not directly refer to a specific title, such as "drama movies", "HBO Tom Hanks comedy movies", and so on. Figure~\ref{fig:entity_statistic_2} shows the proportion of such non-title queries containing different numbers of entities. A significant portion (around 53\%) of the non-title queries contained references to multiple entities, suggesting complex user intents.


% \begin{figure}[ht]
% \centering
% % First image
% \begin{minipage}[b]{0.45\linewidth}
% \includegraphics[width=\linewidth]{Figures/entitites_statistics.pdf}
% \caption{Query-entity distribution on 100K representative queries from search logs}
% \label{fig:entity_statistic}
% \end{minipage}
% \hfill % Optional: add some horizontal spacing
% % Second image
% \begin{minipage}[b]{0.45\linewidth}
% \includegraphics[width=\linewidth]{Figures/entities_statistic_2.pdf}
% \caption{Query-number of entity distribution on non-title representative queries from search logs}
% \label{fig:entity_statistic_2}
% \end{minipage}
% \end{figure}




% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.6\textwidth]{Figures/entitites_statistics.pdf}
% \caption{Query-entity distribution on 100K representative queries from search logs}
% \label{fig:entity_statistic}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[trim=0 0 4cm 0, clip,width=0.6\textwidth]{Figures/entities_statistic_2.pdf}
% \caption{Query-number of entity distribution on non-title representative queries from search logs}
% \label{fig:entity_statistic_2}
% \end{figure}


==> Sections_Hang/Approach.tex <==

 This section illustrates the prompt design technique in our QUS annotation work, which is a combination of the \emph{chain of thought} (CoT) \cite{wei2022chain}, \emph{in-context learning} (ICL) \cite{dong2022survey}, \emph{retrieval-augmented generation} (RAG) \cite{gao2023retrieval}, etc.  The designed prompt is deferred to the appendix due to the space limit.

 \begin{itemize}[leftmargin=*]
 
\item 
\textbf{CoT}.  This is the foundation technique on which our prompt design builds. First, we use CoT across the QUS entities. Notice that the QUS entities are not exclusive, i.e., one query can be multiple QUS entities simultaneously. To avoid the LLM missing some QUS entities, we list each QUS entity's definition and ask an iterative check of each definition. The LLM is required to output all intermediate results. \par Second, we use CoT within each QUS entity. In our experiments, we notice the LLM can make the wrong decisions with minor spelling errors, even if a close example is in the provided in the prompt. One such example is that the LLM \footnote{This phenomenon is observed in the Claude-$2.1$ model.} will regard the \textbf{sell/by/date} and \textbf{sell by date}, \textbf{das} and \textbf{das!}, as different things. Hence, we add some specific rules under the name \emph{Handling Variations and Similarities} to inform the LLM that these queries should be regarded as identical. 



 
\item
\textbf{ICL}. Another technique we use in the prompt design is ICL, as some of the QUS entities may require certain amount of domain knowledge, e.g., \emph{StreamingService}, \emph{OfferType}, \emph{Channel}, \emph{LinearStation}, etc. To help the LLM to properly annotate these QUS entities, we exhaustively search the corresponding examples and append them to the prompt. In addition, we use ICL to help LLM to decide the query similarities, as LLM may make mistakes otherwise. Examples include \textbf{"next time" should be regarded the same as "next time!" with only the exclamation mark}, \textbf{"Romance" should be regarded the same as "romance" with minor differences in capitalized letter}, etc. 

 \item 
 \textbf{RAG}. We observe that it can be challenging for a LLM to determine whether a query is a movie/tv name, which requires a good understanding of the video catalog. To enhance the LLM's capability, we use the RAG approach, i.e., extracting related information with the query and appending it to the prompt. 
 \par 
 As the query is usually of short length, we feel an embedding-based search approach can be an overkill. Instead, we adopt a parameter-free text retrieval approach, which is based on the \emph{normalized compression distance} (NCD) \cite{jiang2023low}. Experiments verify its effectiveness in finding similar movie names and exhibit noticeable improvement in helping LLM  identify the movie/tv names. A brief introduction of this approach can be found in the appendix for the sake of self-containing. 

\item 
\textbf{Miscellaneous.} We let the LLM to assign a confidence score for each of their annotated QUS entity, which helps us in post-processing its annotations. Furthermore, we add some scenario information in the prompt, such as 
\par 
\textbf{consider the use case is that people are looking for movies or TV shows on a streaming service. Hence, bias to relating the search query to the terminologies in the video and entertainment industry,}
\par 
to bias the LLM's decisions towards interpreting the query in the context of streaming service as Prime Video. 
 
\end{itemize}

In addition to the above tasks, we also notice other interesting phenomena 

\begin{itemize}[leftmargin=*]
    \item 
    \textbf{Instructions' location matters.}
We observe that the LLM pays more attention to both ends of prompt. We may improve the labeling performance by simply
moving the important instructions from middle to the front.  This phenomenon is previously observed in \cite{liu2024lost} under the name \emph{lost in the middle}.  In our prompt, we have carefully chosen the positions of each instruction, i.e., begins the prompt with a task summary and ends the prompt with some common mistakes the LLM can make.  

\item 
\textbf{LLM can ignore instructions/examples.} Another attempt in our prompt design is to add examples of LLM conducting annotation job by strictly following our instructions, as we notice the LLM can sometimes skip steps even we specifically ask them to output the middle results. We notice the LLM performance improves with the number of such examples in the beginning but degrades when too many experiments are appended. Preliminary experiments suggest adding too much examples will lead LLM forget about the previous examples. \footnote{One time we asked the LLM to label the query, which is the first example, and found that the LLM made the wrong decision.}
\par 
One potential mitigation is to limit the number of appended examples. For example, we can build a database storing all these examples. For each newly-coming query, we only append the new most similar examples, which is selected via RAG, rather than appending all examples. 
 
\end{itemize}

Having discussed our prompt design for data synthetization, we proceed to to train a model for query understanding, 


 
  

 


==> Sections_Phanideep/hang_approach_refined.tex <==

 This section illustrates the prompt design technique in our QUS annotation work, which is a combination of the \emph{chain of thought} (CoT) \cite{wei2022chain}, \emph{in-context learning} (ICL) \cite{dong2022survey}, \emph{retrieval-augmented generation} (RAG) \cite{gao2023retrieval}, etc.  The designed prompt is deferred to the appendix due to the space limit.

 \begin{itemize}[leftmargin=*]
 
\item 
\textbf{CoT}.  This is the foundation technique on which our prompt design builds. First, we use CoT across the QUS entities. Notice that the QUS entities are not exclusive, i.e., one query can be multiple QUS entities simultaneously. To avoid the LLM missing some QUS entities, we list each QUS entity's definition and ask an iterative check of each definition. The LLM is required to output all intermediate results. \par Second, we use CoT within each QUS entity. In our experiments, we notice the LLM can make the wrong decisions with minor spelling errors, even if a close example is in the provided in the prompt. One such example is that the LLM \footnote{This phenomenon is observed in the Claude-$2.1$ model.} will regard the \textbf{sell/by/date} and \textbf{sell by date}, \textbf{das} and \textbf{das!}, as different things. Hence, we add some specific rules under the name \emph{Handling Variations and Similarities} to inform the LLM that these queries should be regarded as identical. 



 
\item
\textbf{ICL}. Another technique we use in the prompt design is ICL, as some of the QUS entities may require certain amount of domain knowledge, e.g., \emph{StreamingService}, \emph{OfferType}, \emph{Channel}, \emph{LinearStation}, etc. To help the LLM to properly annotate these QUS entities, we exhaustively search the corresponding examples and append them to the prompt. In addition, we use ICL to help LLM to decide the query similarities, as LLM may make mistakes otherwise. Examples include \textbf{"next time" should be regarded the same as "next time!" with only the exclamation mark}, \textbf{"Romance" should be regarded the same as "romance" with minor differences in capitalized letter}, etc. 

 \item 
 \textbf{RAG}. We observe that it can be challenging for a LLM to determine whether a query is a movie/tv name, which requires a good understanding of the video catalog. To enhance the LLM's capability, we use the RAG approach, i.e., extracting related information with the query and appending it to the prompt. 
 \par 
 As the query is usually of short length, we feel an embedding-based search approach can be an overkill. Instead, we adopt a parameter-free text retrieval approach, which is based on the \emph{normalized compression distance} (NCD) \cite{jiang2023low}. Experiments verify its effectiveness in finding similar movie names and exhibit noticeable improvement in helping LLM  identify the movie/tv names. A brief introduction of this approach can be found in the appendix for the sake of self-containing. 

\item 
\textbf{Miscellaneous.} We let the LLM to assign a confidence score for each of their annotated QUS entity, which helps us in post-processing its annotations. Furthermore, we add some scenario information in the prompt, such as 
\par 
\textbf{consider the use case is that people are looking for movies or TV shows on a streaming service. Hence, bias to relating the search query to the terminologies in the video and entertainment industry,}
\par 
to bias the LLM's decisions towards interpreting the query in the context of streaming service as Prime Video. 
 
\end{itemize}

In addition to the above tasks, we also notice other interesting phenomena 

\begin{itemize}[leftmargin=*]
    \item 
    \textbf{Instructions' location matters.}
We observe that the LLM pays more attention to both ends of prompt. We may improve the labeling performance by simply
moving the important instructions from middle to the front.  This phenomenon is previously observed in \cite{liu2024lost} under the name \emph{lost in the middle}.  In our prompt, we have carefully chosen the positions of each instruction, i.e., begins the prompt with a task summary and ends the prompt with some common mistakes the LLM can make.  

\item 
\textbf{LLM can ignore instructions/examples.} Another attempt in our prompt design is to add examples of LLM conducting annotation job by strictly following our instructions, as we notice the LLM can sometimes skip steps even we specifically ask them to output the middle results. We notice the LLM performance improves with the number of such examples in the beginning but degrades when too many experiments are appended. Preliminary experiments suggest adding too much examples will lead LLM forget about the previous examples. \footnote{One time we asked the LLM to label the query, which is the first example, and found that the LLM made the wrong decision.}
\par 
One potential mitigation is to limit the number of appended examples. For example, we can build a database storing all these examples. For each newly-coming query, we only append the new most similar examples, which is selected via RAG, rather than appending all examples. 
 
\end{itemize}

Having discussed our prompt design for data synthetization, we proceed to to train a model for query understanding, 


 
  

 


==> Sections_Phanideep/ranker.tex <==


To evaluate the impact of better query understanding on the retrieval flow, we train a downstream ranker model that takes query intent scores as the input. To assess the effectiveness of enhanced query understanding, the evaluation involves two training scenarios for the Ranker model:

\begin{itemize}
    \item Training the ranker model without any query entities.
    \item Training the ranker using entity distributions from a baseline that is based on lexical matching.
    \item Training the ranker using entity distributions from a BERT-based entity classifier trained using LLM labels as described in the section~\ref{section: multi label model}.
\end{itemize}

\subsubsection{Data}
The model is trained on query-title level clicks and streams from impression logs spanning across 3 weeks. We also train the model on query-title level semantic relevance labels annotated using an LLM based on the query and title metadata. We perform large scale evaluation for engagement on impression data from 4 non consecutive days from a different month than the training. The engagement evaluation data is from the search logs that consists of impression data of around 6k random queries spanning 100k customers where 40\% of the queries were non title searches.

\subsubsection{Experiment Setup}
 The Ranker model is a Multi-Task Learning (MTL) based neural network model used for ranking retrieved items from content providers given a search query. We use a KNN based content provider that fetches relevant titles using lexical and vector embedding criteria. One of the inputs to the ranker model is the probability distributions from the Query Understanding (QU) component apart from query-title and title level features. The model is trained to predict the propensity of clicking and streaming a title given the query, along with predicting the propensity of title being semantically relevant. We use two hidden layers for the shared blocks and one hidden layer for the three tasks with ReLU as the activation function and a learning rate of 5e-4. 
 
\subsubsection{Results}
We evaluate the model for the information retrieval metrics hitrate@1, map@5 (mean average precision) and nDCG@5 (normalised discounted cumulative gain). We report the relative gain of these metrics against the ranker model trained without any query intent signals. 

\begin{table}[h]
    \centering
   \caption{Relative gain in ranker metrics when compared with a model config without the query intent.}
    \begin{tabular}{cccc}
      \toprule
    Model configuration & hitrate@1 & map@5 & nDCG@5 \\
        \hline
        Ranker without query intent & x & x & x \\
        %\hline
        Ranker with lexical baseline & 12\% & 9\% & 8\% \\
        % \hline
        Ranker with multi-label entity classifier & 17\% & 12\% & 11\% \\
        \hline
    \end{tabular}
\end{table}



% \begin{table}[!ht]
% \caption{
% Benchmarking across different LLLMs and prompts. \textbf{Baseline} corresponds to the baseline prompt; \textbf{Baseline + CoT} corresponds to the prompt with CoT technique; and \textbf{Baseline + CoT + ICL} refers to the prompt with both CoT and ICL technique. We mark the best F1, precision, and recall with \blue{\textbf{blue}}, \textbf{black}, and \red{\textbf{red}}, respectively.}
% \vspace{2mm}
% \label{tab:po_kto_dpo}
% \centering
% \resizebox{5.6in}{!}{%
% {\footnotesize
% \begin{tabular}{@{}cccccccccccc@{}}\toprule
% & \multicolumn{3}{c}{\makecell{{Baseline}}} & \phantom{ab}& \multicolumn{3}{c}{\makecell{{Baseline + CoT}}} & \phantom{ab}& \multicolumn{3}{c}{\makecell{{Baseline + CoT + ICL}}}\\
% \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12} 
% & \makecell{F1} & \makecell{Precision} & \makecell{Recall} & & \makecell{F1} & \makecell{Precision} & \makecell{Recall} && \makecell{F1} & \makecell{Precision} & \makecell{Recall}\\  
% (Weighted) \\
% \texttt{Claude-2.1} & $0.8027$ & $0.8785$ & $0.7389$ && $0.8539$ & $0.8985$ & $0.8136$ && $0.8402$ & $0.8282$ & $0.8525$\\
% \texttt{Claude-3} & $0.8122$ & $0.8917$ & $0.7458$ && $0.8585$ & $0.9101$ & $0.8123$ && \blue{$\textbf{0.8719}$} & $\textbf{0.9226}$ & \red{$\textbf{0.8264}$}\\ \\
% (Unweighted) \\
% \texttt{Claude-2.1} & $0.7997$ & $0.8621$ & $ 0.7457$ && $0.8377$ & $0.8511$ & $0.8247$ && $0.8464$ & $0.8336$ & \red{$\textbf{0.8596}$}\\
% \texttt{Claude-3} & $0.8128$ & $0.8696$ & $0.7629$ && $0.8385$ & $0.8760$ & $0.8042$ && \blue{$\textbf{0.8715}$} & $\textbf{0.9251}$ & $0.8238$\\ 
% \bottomrule
% \end{tabular}}
% }
% \end{table}

==> Sections_Rose/Approach.tex <==
\section{Approach}
Our goal is to identify the Intent of Customer search queries. We are first given a dataset $\mathcal{D}_{\mathcal{Q}}$, which consists of abundant customer search queries with labels annotated by LLM. We aim to assign $K$ QUS(Query Understanding) entity candidates, which are restricted to Prime Video use case, to search queries. This is a multi-label classification problem where each customer search query can have multiple tags associated with it. We approach in fine-tuning the pre-trained BERT model with additional classifier layers to handle the multi-labeling task, because it is demonstrated that if large dataset is available, attention-based model should outperform other supervised models.

%\begin{wrapfigure}{r}{0.5\textwidth}
\begin{figure}
    \centering
    \resizebox{0.5\textwidth}{!}
    \includegraphics[width=3 in]{Sections_Rose/AMLC2024_Bert_Structure.png}
    \caption{Natural Language Understanding Model Structure}
    \label{fig:structure}
    \end{figure}
  % \begin{center}
  %   \includegraphics[width=0.48\textwidth]{birds}
  % \end{center}
  % \caption{Birds}
%\end{wrapfigure}



\subsection{BERT-Based Multi-Label Classifier}
Bert is a Transformer based pre-training model trained on Toronto BookCorpus ($800$M words) and English Wikipedia ($2,500$M words). We choose BERT because BERT gives bidirectional contextual representation of each word that is based on the other words in the sentence which is well-known outperforming Context-free models or other unidirectional models. 

In our model setting, we adopt the pre-trained BERT-base model from Hugging Face which has $12$ transformer blocks with $12$ attention heads and $110$ millions parameters. Then we extract the CLS token embedding from the last four hidden layers and concatenate to form sequence representation. Feed it into tag-specific classifiers which consists of two layers neural network followed by sigmoid function to generate the probability for each $K$ QUS entity independently.

\subsection{Data Upsampling/Imbalance}


\subsection{BCE Logistic Loss}
For training, we apply BCE logistic Loss function. This loss combines a Sigmoid layer and the BCELoss in one single class. This loss is more numerically stable than activate sigmoid function followed by the BCELoss because it is taking advantage of log-sum-exp trick to prevent underflow or overflow(TO ADD Formula). And thus, sigmoid activation only be added during the evaluation stage in our setting.


\subsection{Select Best Thresholds for QUS Labels}
F1 measures in the context of classification is well-studied. In our Multi-Label problem, we choose Micro Average to properly captures class imbalances. F1 scores are computed on Evaluation dataset to decide the optimal threshold for each QUS entity. We have seen this significantly improved overall accuracy and entity-wise Precision and Recall metrics. (TODO: Add formula)



==> Sections_Rose/Intent_Classifier_Experiments_Data.tex <==
The proposed Multi-Label Intent Classifier model is trained on a dataset of size 100K which utilize 22 entities to indicate intent of each customer search query. 

==> Sections_Rose/Results.tex <==
\section{Experiment}
\subsection{Data}
100k ground truth data annotated by LLM. QUS entities distribution: TODO. $70\%$ as training dataset,  $10\%$ evaluation dataset,  $20\%$ test dataset. 

\subsection{Experiment Setup}
Optimizer is AdamM, learning rate $=10^{-5}$, epoch 4, batch 32. one GPU: NVIDIA A10G. 

Created checkpoints and calculate evaluation loss after each epoch to select the best model and early stop to save computation.

\subsection{Result}


